SN 2007uy - metamorphosis of an aspheric Type Ib explosion

The supernovae of Type Ibc are rare and the detailed characteristics of these explosions have been studied only for a few events. Unlike Type II SNe, the progenitors of Type Ibc have never been detected in pre-explosion images. So, to understand the nature of their progenitors and the characteristics of the explosions, investigation of proximate events are necessary. Here we present the results of multi-wavelength observations of Type Ib SN 2007uy in the nearby ($\sim$ 29.5 Mpc) galaxy NGC 2770. Analysis of the photometric observations revealed this explosion as an energetic event with peak absolute R band magnitude $-18.5\pm0.16$, which is about one mag brighter than the mean value ($-17.6\pm0.6$) derived for well observed Type Ibc events. The SN is highly extinguished, E(B-V) = 0.63$\pm$0.15 mag, mainly due to foreground material present in the host galaxy. From optical light curve modeling we determine that about 0.3 M$_{\odot}$ radioactive $^{56}$Ni is produced and roughly 4.4 M$_{\odot}$ material is ejected during this explosion with liberated energy $\sim 15\times10^{51}$ erg, indicating the event to be an energetic one. Through optical spectroscopy, we have noticed a clear aspheric evolution of several line forming regions, but no dependency of asymmetry is seen on the distribution of $^{56}$Ni inside the ejecta. The SN shock interaction with the circumburst material is clearly noticeable in radio follow-up, presenting a Synchrotron Self Absorption (SSA) dominated light curve with a contribution of Free Free Absorption (FFA) during the early phases. Assuming a WR star, with wind velocity $\ga 10^3 {\rm km s}^{-1}$, as a progenitor, we derive a lower limit to the mass loss rate inferred from the radio data as $\dot{M} \ga 2.4\times10^{-5}$ M$_{\odot}$, yr$^{-1}$, which is consistent with the results obtained for other Type Ibc SNe bright at radio frequencies.

==> obslog.tex <==
%obslog
%*****************************************************************************
\begin{table}
\caption{Photometric log for SN 2007uy field$^{\dagger}$.}
\label{tab:obslog}
\begin{tabular}{ccccccc}
\hline\hline
Date                      &JD        &Phase  & Exp.time(B band) & Exp.time(V band) &  Exp.time(R band) &  Exp.time(I band)   \\
 (UT)                     &(2454000+)&(days)&  (sec)              & (sec)               & (sec)                & (sec)      \\
\hline
2008 Jan 13.9168          &479.444 &  13.32 &3$\times$300     &2$\times$300     &2$\times$300   &2$\times$300      \\
2008 Jan 14.8336          &480.343 &  14.18 &150              &120              &2$\times$100   &2$\times$80       \\
2008 Jan 15.8753          &481.409 &  15.32 &150, 200         &2$\times$150     &2$\times$100   &100, 120          \\
2008 Jan 29.8338          &495.345 &  29.17 &200, 2$\times$300&200, 300         &100, 200       &2$\times$100      \\
2008 Jan 31.8751          &497.376 &  31.20 &200, 2$\times$300&300, 2$\times$200&2$\times$100   &200, 2$\times$120 \\
2008 Feb 04.8756          &501.382 &  35.21 &2$\times$150     &2$\times$150     &2$\times$100   &100, 200          \\
2008 Feb 09.7084          &506.248 &  40.08 &2$\times$150     &100, 150         &2$\times$100   &80, 100           \\
2008 Feb 15.8336          &512.368 &  46.19 &3$\times$200     &2$\times$200     &$-$            &2$\times$200      \\
2008 Feb 23.6251          &520.132 &  53.98 &3$\times$200     &150, 200, 300    &80, 100        &2$\times$80       \\
2008 Feb 24.5838          &521.117 &  54.95 &$-$              &300              &2$\times$100   &2$\times$150      \\
%2008 Mar 02.7084         &528.242 &  62.08 &2$\times$240     &2$\times$100     &2$\times$100   &2$\times$120      \\
2008 Mar 03.7089          &529.225 &  63.05 &2$\times$240     &2$\times$100     &2$\times$100   &2$\times$120      \\
2008 Mar 05.7922          &531.301 &  65.13 &200, 300         &$-$              &2$\times$100   &100, 150          \\
2008 Apr 29.0000          &586.416 & 120.96 &$-$              &$-$              &5$\times$300   &3$\times$300      \\
2008 Apr 30.6251          &587.134 & 120.96 &$-$              &7$\times$300     &$-$            &$-$               \\
2008 May 02.5835          &589.109 & 122.94 &$-$              &$-$              &900            &$-$               \\
2008 May 05.5835          &592.124 & 125.95 &$-$              &2$\times$900     &$-$            &$-$               \\
\hline
\end{tabular}
\newline\newline
$^{\dagger}$ JD$_{burst}$ = 2454466.16899 (From CBET 1191)\\
%$^{\ast}$ Data taken from IGO, Pune, India
\end{table}
%*****************************************************************************


==> run <==
latex ms
#bibtex ms
#bibtex ms
latex ms
latex ms
#dvips -o ms.ps ms.dvi
dvipdf ms.dvi
\rm *.log
\rm *.aux
\rm *.dvi
#\rm ms.b*
#ps2pdf ms.ps
evince ms.pdf &

